Linear Submodular Maximization with Bandit Feedback

Submodular optimization with bandit feedback has recently been studied in a variety of contexts. In a number of real-world applications such as diversified recommender systems and data summarization, the submodular function exhibits additional linear structure. We consider developing approximation algorithms for the maximization of a submodular objective function $f:2^U\to\mathbb{R}_{\geq 0}$, where $f=\sum_{i=1}^dw_iF_{i}$. It is assumed that we have value oracle access to the functions $F_i$, but the coefficients $w_i$ are unknown, and $f$ can only be accessed via noisy queries. We develop algorithms for this setting inspired by adaptive allocation algorithms in the best-arm identification for linear bandit, with approximation guarantees arbitrarily close to the setting where we have value oracle access to $f$. Finally, we empirically demonstrate that our algorithms make vast improvements in terms of sample efficiency compared to algorithms that do not exploit the linear structure of $f$ on instances of move recommendation.

==> sections/adaptStrategy.tex <==
\subsection{Adaptive Allocation Strategy}
\label{sec:adapt}
% \textcolor{red}{TODO: When computing confidence intervals, do you need to compute a determinant? And if so, are you using the matrix determinant lemma as described by Abbasi-Yadkori et al. for efficient updates?}

% \subsection{Adaptive Allocation Strategy for Linear Bandit}
In the previous part, we present the analysis using the static allocation strategy as the subroutine for \alg in Algorithm \ref{alg:LG} to select the element to be added. However, notice that in Algorithm \ref{alg:LG}, the subroutine algorithm \algsub estimates the same vector $\vect{w}$ in all iterations. Therefore, we can exploit information from past iterations to help select new elements. However, the static allocation strategy cannot be applied to achieve that since the feature vectors (marginal gain vectors) of future iterations depend on the past sampling result, and therefore if we utilize the samples from previous iterations in \alg, the sampling sequence is not independent. In this section, we develop an adaptive allocation algorithm, which is motivated by the algorithm \cite{xu2018fully} and can be adapted to also utilize information from past iterations. Instead of presenting the algorithm directly, we present a more general algorithm \algadapt as described in Algorithm 
\ref{alg:adapt}, which finds the nearly optimal element with an adaptive allocation strategy and also utilizes the offline sampling results.

The input of the algorithm is described as follows: suppose there are two sets of elements: (i). a measurement set containing $m$ elements with features $\vect{x}_1,\vect{x}_2,...,\vect{x}_m$. Furthermore, we assume there is an offline dataset with samples from $\mathcal{X}$; (ii). an evaluation set containing $n$ elements with features $\vect{y}_1,\vect{y}_2,...,\vect{y}_n\in\mR^d$. Here the valuation set $\mathcal{Y}$ can be random but is fixed conditioned on the offline dataset. We denote the sets of features as $\mathcal{Y}=\{\vect{y}_1,...,\vect{y}_n\}$ and $\mathcal{X}=\{\vect{x}_1,...,\vect{x}_m\}$. For each element $i$ with feature $\vect{x}_i$, there are $N_i$ offline samples. The 
$t$-th sampling result of $\vect{x}_i$ is denoted as $R_{i,t}$. The goal of \algadapt is to infer $\arg\max_{a\in[n]}\vect{y}_a^T\vect{w}$ with probability at least $1-\delta$ by making as few noisy samples from $\mathcal{X}$ as possible. Here we denote the optimal element as $a^*=\arg\max_{a\in[n]}\vect{y}_a^T\vect{w}$. In addition, we define $\Delta_i=\vect{y}_{a^*}^T\vect{w}-\vect{y}_i^T\vect{w}$. Next, we describe the proposed algorithm.

The algorithm \algadapt first calculates the covariance matrix $\vect{A}$
and the reward vector $\vect{b}$ corresponds to the sampling history from the offline dataset. Then \algadapt selects elements from the set $\mathcal{X}$ and takes samples to find the element in $\mathcal{Y}$ with the highest expected reward value. 
More specifically, from Line \ref{line:LBAS_for_loop_starts} to Line \ref{line:LBAS_for_loop_ends}, the algorithm initializes by sampling each vector in $\mathcal{X}$ at least once. Then at each round $t$ in the while loop, the agent selects an element $a_t\in[m]=\{1,2,...,m\}$ by the subroutine \selectdir. Here $p_a(i,j)$ in \selectdir is the fraction of samples allocated to element $a$ for measuring the direction of $\vect{y}_i-\vect{y}_j$. From the discussion given in Appendix B in \cite{xu2018fully}, we have that the asymptotic optimal allocation $p^*$ satisfies that 
\begin{align}
\label{eqn:define_p*}
    p_a^*(i,j)=\frac{|w^*_a(i,j)|}{\sum_{a'=1}^m|w^*_{a'}(i,j)|},
\end{align}
 where $\{w^*_{a}(i,j)\}_{a\in[m]}$ is the optimal solution of the linear program in (\ref{eqn:optimization}) below 
\begin{align}
\label{eqn:optimization}
    \arg\min_{\{w_a\}}\sum_{a=1}^m|w_a| \qquad s.t.\qquad \vect{y}_i-\vect{y}_j=\sum_{a=1}^mw_a\vect{x}_a.
\end{align}

Let us further denote $\rho_{i,j}$ as the optimal value of (\ref{eqn:optimization}).


After the element $a_t$ is selected, the stopping condition $B(t)\leq\epsilon$ is checked. If $B(t)\leq\epsilon$ is satisfied, then the element $i_t$ is returned. Otherwise, the algorithm samples $a_t$ and obtains the reward $r_t$ which satisfies 
\begin{align*}  r_t=\vect{x}^T_{a_t}\vect{w}+\epsilon_t.
\end{align*}
 Then $\vect{A}$, $b$, and $T_{a_t}$ are updated and the algorithm proceeds to the next iteration. Here $T_i$ is the number of total samples of the element $i$ with feature $\vect{x}_i$. $\beta_t(i,j)$ is the confidence interval of the direction $\vect{y}_i-\vect{y}_j$ which is defined as $\beta_t(i,j)=C_t||\vect{y}_i-\vect{y}_j||_{\vect{A}_t^{-1}}=(R\sqrt{2\log\frac{\det(\vect{A}_t^{\lambda})^{\frac{1}{2}}\det(\lambda I)^{-\frac{1}{2}}}{\delta}}+\lambda^{\frac{1}{2}}S)||\vect{y}_i-\vect{y}_j||_{\vect{A}_t^{-1}}$. If we set $p_a(i,j)=p_a^*(i,j)$ as defined in (\ref{eqn:define_p*}), we would get the following theorem.
\begin{algorithm}[t]
\caption{\alglongadapt (\algadapt)}\label{alg:adapt}
 \begin{algorithmic}[1]
 \STATE \textbf{Input:}   $\mathcal{X}$, $\mathcal{Y}$, $\epsilon\geq 0$, $\delta>0$
  
 \STATE \textbf{Output: } element $u$
 \STATE  $t\gets 1$
 \STATE  $\vect{A}\gets\sum_{i\in [m]}N_i\vect{x}_i\vect{x}_i^T+\lambda \vect{I}$
 \STATE $\vect{b}\gets\sum_{i\in[m]}\sum_{\tau\in[N_i]}R_{i,\tau}\vect{x}_{i}$
\FOR{$i\in[m]$}\label{line:LBAS_for_loop_starts}
\STATE $T_i\gets N_i$
\IF{$N_i==0$}
\STATE sample $r_t=\vect{x}_i^T\vect{w}+\xi_t$ and obtain the reward $r_t$
\STATE Update $\vect{A}$ and $\vect{b}$
\STATE $t\gets t+1$
\STATE $T_i\gets1$
\ENDIF
\ENDFOR \label{line:LBAS_for_loop_ends}
 \WHILE{\textbf{true}}
 \STATE $a_t\gets$\selectdir$(\vect{A},b,t)$
 \IF{ $B(t)\leq\epsilon$}
  \STATE \textbf{return} $i_t$
 \ENDIF
\STATE sample $r_t=\vect{x}^T_{a_t}\vect{w}+\xi_t$
 \STATE update $\vect{A}$, $\vect{b}$
 \STATE $T_{a_t}\gets T_{a_t}+1$
  \STATE $t\gets t+1$
 \ENDWHILE
 \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{\selectdir($t$)}\label{alg:selectdir}
 \begin{algorithmic}[1]
 \STATE $\hat{\vect{w}}_t=\vect{A}^{-1}\vect{b}$
 \STATE $i_t\gets\arg\max_{i\in[n]}\vect{y}_i^T\hat{\vect{w}}_t$
 \STATE $j_t\gets\arg\max_{j\in[n]}\vect{y}_j^T\hat{\vect{w}}_t-\vect{y}_{i_t}^T\hat{\vect{w}}_t+\beta_t(j,i_t)$
 \STATE $B(t)\gets\vect{y}_{j_t}^T\hat{\vect{w}}_t-\vect{y}_{i_t}^T\hat{\vect{w}}_t+\beta_t(j_t,i_t)$
 \STATE $a_t=\arg\min_{a\in[m]:p_a(i_t,j_t)>0}\frac{T_a}{p_a(i_t,j_t)}$
 \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:adapt}
    With probability at least $1-\delta$, \algadapt in Algorithm \ref{alg:adapt} satisfies that
    \begin{enumerate}
        \item The output element $i$ satisfies that
        \begin{align*}    \vect{y}_i^T\vect{w}\geq\vect{y}_{a^*}^T\vect{w}-\epsilon,
        \end{align*}
        where $a^*=\arg\max_{a\in[n]}\vect{y}_a^T\vect{w}$.
        \item Assume $\lambda\leq\frac{2R^2}{S^2}\log\frac{1}{\delta}$, then the total number of samples $\tau$ of \algadapt satisfies
        \begin{align*}
    \tau&\leq\sum_{a\in[m]}\max\{4\Ha R^2(2\log\frac{1}{\delta}+d\log M)+1-N_a,0\}.
\end{align*}
where $M=\frac{16H_\epsilon R^2L^2}{\lambda}\log\frac{1}{\delta}+\frac{32H_\epsilon^2 R^4L^4}{\lambda^2 }+\frac{2(N+m)L^2}{\lambda d}+2$. Here $H_{\epsilon,a}=\max_{i,j\in[n]}\frac{p_a(i,j)\rho_{i,j}}{\max\{\epsilon,\frac{\Delta_{i}\vee\Delta_{j}+\epsilon}{3}\}^2}$ and $H_{\epsilon}=\sum_{a\in[m]}H_{\epsilon,a}$.
    \end{enumerate}
\end{theorem}

The proof is deferred to Section \ref{appdx:adapt} in the appendix.
Then we describe how we use \algadapt as the subroutine for \alg algorithm. Let us denote the solution set at iteration $l$ in \alg as $S_l$. When \algadapt is invoked at iteration $l$ of \alg, the input measurement set $\mathcal{Y}=\{\vect{y}_1,\vect{y}_2,...,\vect{y}_n\}$ is set to be $\{\Delta\vect{F}(S_l,a)\}_{a\in [n]}$, and the evaluation set $\mathcal{X}$ is set to be $\{\Delta\vect{F}(S_{l'},a)\}_{l'\in[l],a\in[n]}$, which means that the algorithm can sample marginal gain $\Delta f(S_{l'},a)$ for solution set from any past iteration $l'\leq l$ and any element $a\in [n]$. The offline dataset would contain all the noisy samples from the past iterations. Here we denote the total number of samples of $\Delta \vect{F}(S_{l'},a)$ before iteration $l$ as $N_{S_{l'},a}^{(l)}$, and the total number of samples before iteration $l$ as $N^{(l)}=\sum_{l'\in[l],a\in[n]}N_{S_{l'},a}^{(l)}$. Moreover, we define $\Delta_{l,i}=\max_{a\in[n]}\Delta \vect{F}(S_{l},a)^T\vect{w}-\Delta\vect{F}(S_{l},i)^T\vect{w}$. By employing Theorem \ref{thm:adapt}, we can prove the following result on the sample complexity.  
\begin{theorem}
    Suppose \algadapt is used as a subroutine algorithm for \alg, then \alg makes $n$ calls of \algadapt. In addition, with probability at least $1-\delta$, the following statements hold: 
     \begin{enumerate}
    % \vspace{-2mm}
        \item The exact function value of the output solution set $S$ satisfies that $f(S)\geq(1-e^{-1})f(OPT)-\epsilon.$ Here $OPT$ is an optimal solution to the SM problem;
         
        \item Each call of \algadapt at iteration $l$ takes samples $\tau_l$ that satisfies
    \begin{align*}
    \tau_l&\leq\sum_{l'\in[l],a\in[n]}\max\{4H^{(l)}_{l',a} R^2(2\log\frac{\kappa}{\delta}+d\log M^{(l)})+1-N_{S_{l'},a}^{(l)},0\}.
\end{align*}
    where $M^{(l)}=\frac{16H_\epsilon^{(l)} R^2L^2}{\lambda}\log(\frac{\kappa}{\delta})+\frac{32(H_\epsilon^{(l)})^2 R^4L^4}{\lambda^2 }+\frac{2(N^{(l)}+n(l-1))L^2}{\lambda d}+2$. Here $H_{l',a}^{(l)}=\max_{i,j\in[n]}\frac{p_a(i,j)\rho_{i,j}}{\max\{\epsilon/\kappa,\frac{\Delta_{l,i}\vee\Delta_{l,j}+\epsilon/\kappa}{3}\}^2}$ and $H_{\epsilon}^{(l)}=\sum_{l'\in[l],a\in[n]}H_{l',a}^{(l)}$.
   % Besides, it holds with probability $1$ that 
    % where $\epsilon=3\epsilon$. 
    \end{enumerate}
\end{theorem}



==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    % \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the main claims made in the abstract and introduction of the paper accurately reflect the paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper discusses the limitations of the work performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, for each theoretical result, the paper provides the full set of assumptions and a complete proof.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper fully discloses all the information needed to reproduce the main experimental results of the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiment results can be easily reproduced by the given pseudocodes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper specifies all the relevant parameters.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper provides the significant statistics of our experiments. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper provides the details on the computing resources. 
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper conforms in every respect with the NeurIPS Code of Ethics. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we address the potential broader impacts in the appendix. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not introduce new datasets in this paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Yes, all assets used in this paper have been properly cited. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no assets released.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/figures/stream.tex <==
\vspace{-1em}
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.7]

\draw (0,0) to (9,0);
\draw node at (10,1) {$w+\epsilon$};
\draw node at (10,0) {$w$};
\draw node at (10,-1) {$w-\epsilon$};
\draw[thick,dotted,red] (0,1) to (9,1);
\draw[thick,dotted,red] (0,-1) to (9,-1);

\draw[thick,cyan,->] (1,0.5) to (1,2);
\draw[thick,cyan,->] (1,0.5) to (1,-1);
\draw[cyan,fill=cyan] (1,0.5) circle [radius=0.1];
\draw node at (1.5,0.5) {$(a)$};

\draw[thick,cyan,->] (3,-0.5) to (3,1);
\draw[thick,cyan,->] (3,-0.5) to (3,-2);
\draw[cyan,fill=cyan] (3,-0.5) circle [radius=0.1];
\draw node at (3.5,-0.5) {$(b)$};

\draw[thick,cyan,->] (5,0.5) to (5,2.5);
\draw[thick,cyan,->] (5,0.5) to (5,-1.5);
\draw[cyan,fill=cyan] (5,0.5) circle [radius=0.1];
\draw node at (5.5,0.5) {$(c)$};

\draw[thick,cyan,->] (7,0) to (7,1);
\draw[thick,cyan,->] (7,0) to (7,-1);
\draw[cyan,fill=cyan] (7,0) circle [radius=0.1];
\draw node at (7.5,0.5) {$(d)$};

%  \draw [cyan, fill=cyan] (13,0) circle [radius=0.25];
%  \draw [cyan, fill=cyan] (11,0) circle [radius=0.25];
%  \draw [dotted, thick] (6,0) to (9,0);
%  \draw node at (8,-1.5) {\scriptsize Discarded elements};


%\draw (17,0) ellipse (3cm and 6cm);
%\draw [cyan, fill=cyan] (15,2.5) circle [radius=0.25];
%\draw [cyan, fill=cyan] (18,-0.5) circle [radius=0.25];
%\draw [cyan, fill=cyan] (19,1.5) circle [radius=0.25];
%\draw [cyan, fill=cyan] (17.5,1) circle [radius=0.25];
%\draw [cyan, fill=cyan] (16,-3) circle [radius=0.25];
%\draw [cyan, fill=cyan] (15.5,-1.5) circle [radius=0.25];
%\draw (17,-7.5) node {\scriptsize$U'$};


%\draw [WildStrawberry,thick,-{Latex[length=2mm,width=2mm]}] (24,0) to (21,0);
%\draw [cyan, fill=cyan] (25,0) circle [radius=0.25];
%\draw [cyan, fill=cyan] (26,0) circle [radius=0.25];
%\draw [cyan, fill=cyan] (27,0) circle [radius=0.25];
%\draw [cyan, fill=cyan] (28,0) circle [radius=0.25];
%\draw [dotted, thick] (33,0) to (30,0);
%\draw node at (27,-1.5) {\scriptsize Elements from $U$ arrive};

\end{tikzpicture}
\caption{An illustration of the various states of \samp. The blue dots depict the values of $\widehat{\Delta f_t}(S,u)$, while the surrounding blue lines depict the confidence region $[\widehat{\Delta f_t}(S,u)-C_t, \widehat{\Delta f_t}(S,u)+C_t]$. Once the region looks like (a), \samp will return true. In (b), \samp will return false. In (c), \samp will continue sampling to reduce the width of the confidence region. Finally, in (d) \samp has taken $N_2$ samples resulting in an $\epsilon$-approximation.}
\label{fig:samp}
\end{figure}


==> sections/theoretical.tex <==

\section{The Standard Greedy Algorithm with Linear Bandit Feedback}
\label{sec:greedy}

\textcolor{red}{I think we should actually combine all the pseudocode into one algorithm. The reason for this is there are so many updates of the same variables that the input/output format is misleading. In the text, we can describe the line numbers of each part of the computation (e.g. say the select direction part of the pseudocode is lines ...}
In this section, we first propose and analyze a greedy algorithm for SM in the linear bandit setting. In particular, our algorithm \alglong (\alg) is based on the standard greedy algorithm (described further in the related work \textcolor{red}{make sure we describe what the standard greedy algorithm is}). Like the standard greedy algorithm, \alg proceeds in a series of $\kappa$ rounds where during each round a single element is added to the solution. But instead of identifying the element of $U$ with the maximum marginal gain to $f$ at each round, \alg invokes the subroutine \algsub to select the element with approximately the highest marginal gain \textcolor{red}{with high probability} using techniques designed specifically for the linear bandit setting. We focus in the main text on an adaptive strategy where decisions are made based on the outcome of previous noisy queries, but an alternative static strategy is presented in the appendix. \textcolor{red}{I think it may make sense to reference the static in the main paper but entirely include it in the appendix.}

Identifying the element with the highest marginal gain reduces to the problem of best-arm identification in linear bandits. Therefore \algsub could be replaced by any existing algorithm for best-arm identification in linear bandit, with some adjustments made to the overall theoretical guarantees. One big difference for our setting is that we do not just have a single round of multi-armed bandit but rather a series of rounds (one round per element chosen into our solution set). While it is possible to simply use an existing best-arm identification strategy at each round, there is potential for a better algorithm since in the greedy algorithm we have a history of rounds before the current one which have also yielded information. Our algorithms is inspired by the best-arm-identification algorithm of \cite{xu2018fully}, but takes advantage of this new setting in a number of ways. \textcolor{red}{This new setting presents technical challenges because ...}. 
%However, the \algsub that we propose in this paper is distinct from those approaches because \textcolor{red}{talk about reasons why our alg is a novel contribution}.
We now state Theorem \ref{thm:greedy}, which is the main theoretical guarantee of our algorithm \alg. 
%The algorithm takes the additive error parameter $\epsilon$, error probability $\delta$ as input. At each iteration, \alg invokes the subroutine algorithm \algsub to select the element with approximately the highest marginal gain and add to the solution set $S$. 
% since $\vect{w}$ is unknown, we use some algorithm for best-arm identification (pure exploration) in the linear bandit literature to select an element. Then once an element with high marginal gain is found we greedily add the element to the solution set. 
%The proposed algorithm \alglong (\alg) is presented in Algorithm \ref{alg:LG}. With the assumption that the subroutine algorithm \algsub finds the element with the highest marginal gain within an $\epsilon/\kappa$ additive error, the output solution returned by \alg satisfies the following Theorem \ref{thm:greedy}.
\textcolor{red}{I guess the first sentence you have in the below theorem is so that we could put in different \algsub algs, but I think it's better to mention that in the \algsub section (in particular that you could replace \algsub with some other best arm id alg that returns a solution such that ...}
\begin{theorem}
\label{thm:greedy}
    %If the output element $u$ of the subroutine algorithm \algsub in Algorithm \ref{alg:LG} satisfies that $\Delta f(S,u)\geq\max_{s\in U}\Delta f(S,s)-\epsilon/\kappa$ with probability at least $1-\delta/\kappa$ , then it follows that
    Algorithm \ref{alg:LG} returns a solution set $S$ that satisfies with probability at least $1-\delta$ then 
    \begin{align*}
        f(S)\geq(1-e^{-1})f(OPT)-\epsilon.
    \end{align*}
\end{theorem}

\textcolor{red}{Need to define OPT somewhere.}
One may see from Theorem \ref{thm:greedy} that \alg achieves the same quality of solution as the standard greedy algorithm with high probability. In the remainder of this section, we describe our algorithms \alg and \algsub and provide a theoretical analysis leading up to the result stated in Theorem \ref{thm:greedy}. In particular, \textcolor{red}{describe what each section is, may need to do this later because we might change the section.}

%The proof is similar to that of Theorem 1 in \cite{singla2016noisy} and we omit it here. Notice that for each $S\subseteq U$ and each element $s\in U$, the noisy marginal gain can be denoted as $\widetilde{\Delta f}(S,s)=\Delta \vect{F}(S,s)^T\vect{w}+\xi$, which satisfies the linear model.
%Thus, identifying the element with the highest marginal gain reduces to the problem of best-arm identification in linear bandits. Consequently, any best-arm identification algorithm in linear bandits can serve as a subroutine for \alg. In the following part, we introduce two types of algorithms in linear bandit literature under the pure exploration setting. We then describe how these algorithms can be adapted as subroutines for \alg. Before we proceed to present the two algorithms, first we present the estimation of the weight vector $\vect{w}$ in linear bandit.


\subsection{Selecting Arms to Sample}
\textcolor{red}{If we can sample from past arms, maybe we should change the definition of the bandit in the preliminaries to be some number of arms $m$ instead of $n$. I may have been describing it earlier as the arms corresponding to the ground set, but maybe this is misleading.}
Instead of greedily selecting the element of maximum marginal gain to add in to our solution by directly querying the objective $f$ (which we do not have oracle access to in our noisy setting), we employ a best-arm identification strategy in order to find the element of approximately maximum marginal gain in as few noisy samples as possible. In particular, we replace the problem of finding $u\in U$ such that $\Delta f(S,u)\geq \max_{x\in U}\Delta f(S,x)$ from the standard greedy algorithm into the linear bandit setting as the problem of finding an arm $\hat{a}$ that satisfies $\vect{x}^T_{\hat{a}}\vect{w}\geq\max_{a\in [n]}\vect{x}^T_{a}\vect{w}-\epsilon'$ where $\epsilon'=\epsilon/\kappa$. The problem is now deciding which arms to pull so that we may shrink our confidence interval stated in from Proposition 1 such that we have found the solution to this problem in as few pulls as possible \textcolor{red}{check whether this sentence makes sense}. Let the optimal element be $a^*=\arg\max_{a\in[n]}\vect{x}_a^T\vect{w}$. \textcolor{red}{I think we should put the static algorithm in the supplementary as well, and just reference the fact that it is in the appendix.}
%In the following sections, we present two algorithms for pure exploration in linear bandit, which include the static allocation algorithm \algstat and the adaptive allocation algorithm \algadapt. Throughout the subsequent sections, we define some notations. 
% In addition, we define the gap of the expected reward of element $i$ and $j$ as $\Delta_{i,j}$, i.e., $\Delta_{i,j}=\vect{x}_i^T\vect{w}-\vect{x}_j^T\vect{w}$.

\textcolor{red}{Need to be more clear at this point what these various inputs are, since this is the first time we are really describing our setup that much.}
We now describe an algorithm to choose what arm to sample in order to find the desired arm as quickly as possible. Suppose we have the following: (i) a measurement set containing $m$ elements with features $\vect{x}_1,\vect{x}_2,...,\vect{x}_m$ \textcolor{red}{Is the measurement set all past arms that have been pulled (with repetition)? Not clear at this point what the set refers to}, (ii) an offline dataset with samples from $\mathcal{X}$ \textcolor{red}{It's also not clear what this is at this point, should be more clear, it is all past sample outcomes?}, (iii) an evaluation set containing $n$ elements with features $\vect{y}_1,\vect{y}_2,...,\vect{y}_n\in\mR^d$ \textcolor{red}{Are these the elements of the ground set $U$?}. Here the valuation set $\mathcal{Y}$ can be random but is fixed conditioned on the offline dataset. We denote the sets of features as $\mathcal{Y}=\{\vect{y}_1,...,\vect{y}_n\}$ and $\mathcal{X}=\{\vect{x}_1,...,\vect{x}_m\}$. For each element $i$ with feature $\vect{x}_i$, there are $N_i$ offline samples. The 
$t$-th sampling result of $\vect{x}_i$ is denoted as $R_{i,t}$. The goal of \algadapt is to infer $\arg\max_{a\in[n]}\vect{y}_a^T\vect{w}$ with probability at least $1-\delta$ by making as few noisy samples from $\mathcal{X}$ as possible. Here we denote the optimal element as $a^*=\arg\max_{a\in[n]}\vect{y}_a^T\vect{w}$. In addition, we define $\Delta_i=\vect{y}_{a^*}^T\vect{w}-\vect{y}_i^T\vect{w}$. Next, we describe the proposed algorithm.

The algorithm \algadapt first calculates the covariance matrix $A$
and the reward vector $\vect{b}$ corresponds to the sampling history from the offline dataset. Then \algadapt selects elements from the set $\mathcal{X}$ and takes samples to find the element in $\mathcal{Y}$ with the highest expected reward value. 
More specifically, from Line \ref{line:LBAS_for_loop_starts} to Line \ref{line:LBAS_for_loop_ends}, the algorithm initializes by sampling each vector in $\mathcal{X}$ at least once. Then at each round $t$ in the while loop, the agent selects an element $a_t\in[m]=\{1,2,...,m\}$ by the subroutine \selectdir. Here $p_a(i,j)$ in \selectdir is the fraction of samples allocated to element $a$ for measuring the direction of $\vect{y}_i-\vect{y}_j$. From the discussion given in Appendix B in \cite{xu2018fully}, we have that the asymptotic optimal allocation $p^*$ satisfies that 
\begin{align}
\label{eqn:define_p*}
    p_a^*(i,j)=\frac{|w^*_a(i,j)|}{\sum_{a'=1}^m|w^*_{a'}(i,j)|},
\end{align}
 where $\{w^*_{a}(i,j)\}_{a\in[m]}$ is the optimal solution of the linear program in (\ref{eqn:optimization}) below 
\begin{align}
\label{eqn:optimization}
    \arg\min_{\{w_a\}}\sum_{a=1}^m|w_a| \qquad s.t.\qquad \vect{y}_i-\vect{y}_j=\sum_{a=1}^mw_a\vect{x}_a.
\end{align}

%Instead of presenting the algorithm directly, we present a more general algorithm \algadapt as described in Algorithm \ref{alg:adapt}, which finds the nearly optimal element with an adaptive allocation strategy and also utilizes the offline sampling results.

\begin{algorithm}[t]
\caption{\alglong (\alg)}\label{alg:LG}
 \begin{algorithmic}[1]
 \STATE \textbf{Input:} $\delta, \epsilon$
 % \STATE  Define $\epsilon':=\frac{\epsilon}{6\kappa}$
 \STATE \textbf{Output: } solution set $S\subseteq U$
 
 \STATE  $S\gets \emptyset$
 \FOR{$j=1,...,\kappa$}
 \STATE $u=\algsub(\Delta \vect{F}, S, \epsilon,\frac{\delta}{\kappa})$
 \STATE $S=S\cup \{u\}$
 \ENDFOR
 \STATE \textbf{return} $S$
 \end{algorithmic}
\end{algorithm}




%\subsubsection{Warm-up: static allocation strategy}
%\label{sec:static}
%The first subroutine algorithm is \algstat, which is presented in Algorithm \ref{alg:static} in the Appendix. The strategy is static in that the sequence of $\vect{x}_i$ is independent from the sampling results. The algorithm is based on the static allocation algorithm proposed in \cite{soare2014best}, which finds the exact optimal solution. Here we develop an algorithm that finds the element with the highest marginal gain within an $\epsilon$ additive error. The theoretical guarantee is stated below. 
%\begin{theorem}
%\label{thm:static}
%    With probability at least $1-\delta$, the Algorithm \ref{alg:static} selects the element $i$ that satisfies
%    \begin{align}
    % \label{eqn:top_mar_gain}
%        \vect{x}^T_i\vect{w}\geq \max_{i\in [n]}\vect{x}^T\vect{w}-\epsilon
%    \end{align}
%    Besides, the number of samples required by invoking \algstat$(S,\epsilon,\delta)$ is upper bounded by $$t\leq\max\{\frac{256R^2d}{\max\{\Delta_{\min}^2,\epsilon^2\}}\log(\frac{256R^2d\pi n}{\max\{\Delta_{\min}^2,\epsilon^2\}}\sqrt{\frac{1}{3\delta}}),\frac{d+d^2+2}{2}\} $$
%    where $\Delta_{\min}=\min_{\{j\in [n],j\neq a^*\}}\vect{x}_{a^*}^T\vect{w}-\vect{x}_j^T\vect{w}$.
%\end{theorem}
% Here $\beta$ is an approximation parameter resulting from converting the continuous solution of the LP problem to a discrete solution.
%The main proof of this Theorem is deferred to Section \ref{appdx:static} in the appendix.



% \section{Exploitation from previous samples}
% From Algorithm \ref{alg:LG}, we can see that for each greedy round, the algorithm invokes Algorithm \ref{alg:static} to estimate the same unknown vector $\vect{w}$. An intuitive question would be: can we use the previous sampling result to find the best element and help improve the sample complexity? Notice that the marginal gain vectors depend on the sampling results in the past greedy iterations and are thus not independent of the estimate of $\hat{\vect{w}}^{(j)}$ from any previous iteration $j$. Therefore, at any iteration $i$, we can't use the estimate of parameter $\hat{\vect{w}}^{(j)}$ 
% from any previous round $j$ where $j<i$ to bound $|(\vect{x}^{(i)})^T(\hat{\vect{w}}^{(j)}-\vect{w})|$.
%  However, we can use the concentration inequality from Proposition \ref{prop:adaptive} to help eliminate the sub-optimal arms. We use $\vect{A}^{(i)}$ and $\hat{\vect{w}}^{(i)}$ to denote the matrix $A$ and the estimate of parameters $\vect{w}$ when the subroutine algorithm \algstat completes greedy iteration $i$. We also use $\vect{x}^{(i)}:=\Delta \vect{F}(S^{(i)},x)$ to represent the marginal gain vector of adding the element $x$ to the solution set $S^{(i)}$. Then it follows that by the concentration inequality, we have that with probability at least $1-\frac{\delta}{2k}$, 
%  \begin{align}
%      |\vect{x}^T(\tilde{\vect{w}}-\vect{w})|\leq C^{(j)}||\vect{x}||_{\vect{A}^{-1}}.
%  \end{align}



% \begin{algorithm}[t]
% \caption{\alglonge (\alge)}\label{alg:LG_eln}
%  \begin{algorithmic}[1]
%  \STATE \textbf{Input:} $\delta, \epsilon$
%  % \STATE  Define $\epsilon':=\frac{\epsilon}{6\kappa}$
%  \STATE \textbf{Output: } solution set $S$
 
%  \STATE  $S\gets \emptyset$
%  \STATE $A\gets\vect{0}_{d\times d}$
%  \STATE $\vect{b}\gets\vect{0}_{d\times 1}$
%  \FOR{$j=1,...,k$}
%  \STATE $B\leftarrow U$
%  \FOR{ $x\in U$}
%  \IF{ $\exists x'\in U$, $C_j||\Delta \vect{F}(S,x)-\Delta \vect{F}(S,{x'})||_{\vect{A}^{-1}}\leq (\vect{x}- \vect{F}_{x'})^T\tilde{\vect{w}}+\epsilon$}
%   \STATE $B\leftarrow B/\{x\}$
%  \ENDIF
%  \ENDFOR
%  \IF{$|B|\leq d$} \STATE $(\vect{A}^{(j)},\vect{b}^{(j)},u)=\texttt{EXP-GREEDY}(S,B,\epsilon,\frac{\delta}{k})$
%  \ELSE \STATE 
% $(\vect{A}^{(j)},\vect{b}^{(j)},u)=\algstat(\Delta \vect{F}, S, B, \epsilon,\frac{\delta}{k})$
% \ENDIF
%  \STATE $S\gets S\cup \{u\}$
%  \STATE \label{line:update_A} $A\gets A+\vect{A}^{(j)}$
%  \STATE \label{line:update_b} $\vect{b}\gets \vect{b}+\vect{b}^{(j)}$
%  \STATE $\tilde{\vect{w}}\gets \vect{A}^{-1}\vect{b}$
%  \ENDFOR
%  \STATE \textbf{return} $S$
%  \end{algorithmic}
% \end{algorithm}



% % For notation simplicity, we denote the vector $\Delta \vect{F}(S_t,s_t)$ as $\vect{x}_t$. We define matrix $\vect{X}_t=todo$ and vector $\vect{b}$. By definition, we know that $\Delta f_t(S_t,s_t)=\vect{x}_t^T\vect{w}+\xi_t$. The least-square error function is 
% % \begin{align}
% %     L(\vect{X},\vect{b};\vect{w})=\sum_{\tau=1}^t(\Delta f_\tau(S_\tau,s_\tau)-\vect{x}_\tau^T\vect{w})^2=(\vect{b}_t-\vect{X}_t\vect{w})^T(\vect{b}_t-\vect{X}_t\vect{w}).
% % \end{align}
% % If we take derivative of the function $ L(\vect{X},\vect{w})$ with respect to $\vect{w}$, and solve $\frac{\partial L(\vect{X},\vect{w})}{\partial \vect{w}}=0$, we can obtain the least squares estimation of parameter $\vect{w}$.
% % \begin{align}
% %     \hat{\vect{w}}_t=(\vect{X}_t^T\vect{X}_t)^{-1}\vect{X}_t^T\vect{b}_t.
% % \end{align}

% % Since the matrix $\vect{X}_t^T\vect{X}_t$ can be inconvertible in some problem instances, the regularized least-square estimate is also used.
% % \begin{align}
% %     \hat{\vect{w}}_t^{\lambda}=(\vect{X}_t^T\vect{X}_t+\lambda \vect{I})^{-1}\vect{X}_t^T\vect{b}_t.
% % \end{align}

% We have the following concentration inequalities 

